Natural Language Does Not Emerge 'Naturally' in Multi-Agent Dialog

A number of recent works have proposed techniques for end-to-end learning of communication protocols among cooperative multi-agent populations, and have simultaneously found the emergence of grounded human-interpretable language in the protocols developed by the agents, all learned without any human supervision! In this paper, using a Task and Tell reference game between two agents as a testbed, we present a sequence of 'negative' results culminating in a 'positive' one -- showing that while most agent-invented languages are effective (i.e. achieve near-perfect task rewards), they are decidedly not interpretable or compositional. In essence, we find that natural language does not emerge 'naturally', despite the semblance of ease of natural-language-emergence that one may gather from recent literature. We discuss how it is possible to coax the invented languages to become more and more human-like and compositional by increasing restrictions on how two agents may communicate.

==> sections/main/all_examples_figure.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
    \centering
    \begin{subfigure}{0.95\linewidth}
	\includegraphics[width=\columnwidth]{figures/examples_sec41_supp.png}\\
    \caption{
    \sk{Overcomplete vocabularies setting ($|V_Q| = |V_A| =64$, \refsec{sec:overcomplete}).
    Owing to a large vocabulary, we denote the tokens using numbers, as opposed to English alphabet characters shown in other figures.
    The learnt mapping is highly non-human intuitive and non-compositional.}}
    \label{fig:ex_overcomplete}
    \end{subfigure}\\
    \vspace{20pt}
    \begin{subfigure}{0.95\linewidth}
    \includegraphics[width=\columnwidth]{figures/examples_sec42_supp.png}\\
    \caption{
    \sk{Attribute and Value vocabulary setting ($|V_Q| = 3, |V_A| = 12$, \refsec{sec:Mem-L}).
    We show symmetric tasks for each instance on either side to illustrate the similarities in the language between the agents.
    As seen here, \Qbot maps symmetric tasks in an order-agnostic fashion, and uses only the first token to convey task information to \Abot.}}
    \label{fig:ex_attribute_vocab}
    \end{subfigure}\\
    \vspace{5pt}
    \caption{Example agent dialogs for the overcomplete and attribute-value vocabulary settings. Green and red nodes correspond to utterance by \Qbot and \Abot respectively.}
%\vspace*{-80pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/main/all_scenario_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
	\centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{c c c c c c c}
    	\toprule
    	\multirow{2}{*}{Setting} 
    	& \multicolumn{2}{c}{Vocab.} 
        & \multicolumn{2}{c}{Memory} 
        & \multicolumn{2}{c}{Gen.(\%)}\\
    
    & \textbf{$V_Q$} & \textbf{$V_A$} & A & Q & Both & One\\ \midrule
        
        Overcomplete (\S\ref{sec:overcomplete}) & 64 & 64 & \cmark & \cmark & 25.6 & 79.5 \\
		Attr-Value (\S\ref{sec:Mem-L}) & 3 & 12 & \cmark & \cmark & 38.5 & 88.4\\
        %NoMem-L (\FIXME{ref}) & 3 & 12 & \xmark & \cmark & 44.9  & 96.2\\
        %Mem-Min (\FIXME{ref}) & 3 & 4 & \cmark & \cmark & 41.0  & 89.7\\
        NoMem-Min (\S\ref{sec:nomem_min}) & 3 & 4 & \xmark & \cmark & \textbf{74.4} & \textbf{94.9}\\ 		\bottomrule
    \end{tabular}}
    \caption{Overview of settings we explore to analyze the language learnt by two agents in a cooperative game, \tnt. Last two columns measure generalization in terms of prediction accuracy of \textbf{both} or at least \textbf{one} of the attribute pair, on a held-out test set containing unseen instances. 
    %Higher the better.
    }
    \label{tab:overview-setting}
    %\vspace*{-11pt}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}
% 	\centering
%     \begin{tabular}{c c c c c c c c}
%     	\multirow{2}{*}{Setting} 
%     	& \multicolumn{2}{c}{Vocab.} 
%         & \multicolumn{2}{c}{Memory} 
%         & \multirow{2}{*}{Gen.}
%         & \multirow{2}{*}{Pros}
%         & \multirow{2}{*}{Cons}\\
    
%     & \textbf{$V_Q$} & \textbf{$V_A$} & \Abot & \Qbot &&&\\ \hline
%         Overcomplete (theory) & 6 & 64 & \cmark & \cmark & 0.0\% & blah & blah\\
% 		Large (Sec.\FIXME{ref}) & 6 & 12 & \cmark & \cmark & 24.4\% & blah & blah \\
%         NoMem-Large (Sec.\FIXME{ref}) & 6 & 12 & \xmark & \cmark & xxx & blah & blah \\
%         Mem-Minimal (Sec.\FIXME{ref}) & 3 & 4 & \cmark & \cmark & xxx & blah & blah \\
%         NoMem-Minimal (Sec.\FIXME{ref}) & 3 & 4 & \xmark & \cmark & xxx & blah & blah \\
%         NoMem-Both-Large (Sec.\FIXME{ref}) & 12 & 6 & \xmark & \xmark & xxx & blah & blah \\ \hline
%     \end{tabular}
%     \caption{\FIXME{An overview of all the settings, details in each setting}}
%     \label{tab:overview-setting}
% \end{table*}

==> sections/main/experiments.tex <==
\vspace{\sectionReduceTop}
\section{The Road to Compositionality}
\label{sec:game-config}
\vspace{\sectionReduceBot}

\begin{figure*}
	\centering
    \includegraphics[width=0.8\textwidth]{figures/language_chart_v2.png}
    \includegraphics[width=0.18\textwidth]{figures/main_examples_v1.png}
    \caption{\FIXME{Detailed caption, figure might change, added to estimate space. Observations are mentioned here, and not in the text in the interest of space.}
    \FIXME{Also state that image->language link breaks down during unseen images. Show negative examples if we are talking about it.}}
    \label{fig:lang_chart}\vspace{-11pt}
\end{figure*}

\ad{
    Compositionality in language does not emerge without the need for it.
    If multiple optimal policies are attainable, the model picks policies that are easier to learn
    \eg given a large vocabulary, the model enumerates all possible instances, than learn to compose instances as
    combinations of individual attributes~\cite{visdial_rl}.
}
\sk{
    % We argue that compositionality in language does not emerge without the need for it.
    % In other words, the model does not necessarily pick an compositional policy if there are other equally optimal uninterpretable policies.
    In this section, we present a series of settings that get progressively restrictive and coax the agents towards adopting a compositional language.
    We also provide insights along the way that help us naturally transition into subsequent settings.
}
\sml{
    For each setting, we provide qualitative analysis
    of the learned languages and report on their ability to generalize to unseen instances.
    We use 80\% of the instances for training and the remaining 20\% to evaluate these learned policies.
}
\vspace{\subsectionReduceTop}
\subsection{Over-Complete Vocabularies}
\label{sec:overcomplete}
\vspace{\subsectionReduceBot}

\sk{
    We begin with the discussion on large vocabularies $V_A$ and $V_Q$ for the agents.
    For instance, if the \Abot vocabulary $|V_A| \ge 64$ (\ad{\#instances}), the optimal policy learnt simply ignores what \Qbot asks and \Abot conveys the entire instance in a single token (\eg token $1 \equiv $ \emph{(red, square, filled)}).
    As one would expect, such a policy \ad{that is not compositional} would have poor generalization to unseen instances.
}
\ad{
    This is similar to the finding in~\cite{visdial_rl}.
    As with human communication, a limited vocabulary that cannot possibly encode the richness of the instance is necessary for non-trivial dialog to emerge.
}
\sk{
    Hence, we would need to restrict $|V_A|$ to be smaller than the number of instances, and represent the number of concepts, \ie., number of attributes $12$.
    We discuss this next.
}

\input{sections/main/all_scenario_table.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{\subsectionReduceTop}
\subsection{Concept Vocabulary}
\vspace{\subsectionReduceBot}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We note that for the task setting presented above (with purely dialog-dependent prediction), has more tokens than the number of images.
\ad{
    We restrict $|V_A|$ to ground it in the number of attributes, \ie, $|V_A| = 12$, and
    analogously $|V_Q| = |\{N, O, \cdots, Z\}| = 12$.
}
% \Qbot and \Abot require 3 and 4 tokens respectively in order to fully solve this task. We argue this simply by observing
% that for $|V_Q| < 3$, there are at most 4 unique utterance pairs over two rounds of dialog while there are 6 possible
% tasks to be communicated. Similarly, without at least $|V_A| = 4$, \Qbot cannot fully specify attribute values.
% In this section, we consider a setting where agents have an over-complete vocabulary consisting of 12 tokens
% per bot, \ie. $|V_A| = |V_Q| = 12$.

\noindent
\textbf{Observations.}
\sk{
    We find that the resulting language is not compositional and is difficult to interpret.
    Following are two salient observations:
}

\sk{
    First, we observe that \Qbot only seems to use the first round of interaction to convey the required pair of attributes to \Abot (and the second round utterance does not seem to obey a pattern).
    Since $|V_Q| > 6$, \Qbot simply assigns one token to each task, \eg, the tasks \emph{(color, shape), (shape, color)} always elicit the tokens \emph{X} and \emph{Y} respectively, from \Qbot in the first round, while the second round is inconsistent across instances for the same task.
    Refer supplement for complete task encodings.
}

\sk{
    Second, as a consequence of this `1-round task-encoding' behavior of \Qbot, the replies from \Abot are not compositional across rounds.
    Specifically, \Abot learns one out of several possible task-dependent mappings from attribute pairs ($4 \times 3 = 12$) to token pairs across rounds ($12 \times 12 = 144$).
    Owing to a large number of possible policies, compositionality is rare in this case, as expected.
    To counter this behavior, we:
    (a) limit $|V_A|$ to minimal size needed to accomplish the task,
    (b) make \Abot memoryless to obtain consistent grounding to \Abot's responses across rounds.
    In particular, we \ad{fix} $|V_A|=4$, and let \Abot's answer $a_t$ to the question $q_t$ be independent of $S^A_{t-1}$, at a given round $t$.
}
% \FIXME{Mention that $|V_A|=12$ is in supplement.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The trends are difficult to analyze, can go to supplement
% and mention a line here.
%\subsection{Memoryless \Abot, Large Vocabulary}
%\label{sec:toy_alt_task_state}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\FIXME{Remove this in the interest of space. Can go into supplementary. We could not even figure out what the agents were doing.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{\subsectionReduceTop}
\subsection{Memoryless \Abot, Minimal Vocabulary}
\label{sec:toy_alt_task_state}
\vspace{\subsectionReduceBot}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\sk{
    For the task setting presented above,
    \Qbot and \Abot require 3 and 4 tokens respectively in order to \ad{succeed at} this task.
    We argue this simply by observing that for $|V_Q| < 3$, there are at most 4 unique utterance pairs over two rounds of dialog while there are 6 possible tasks to be communicated.
    Similarly, without at least $|V_A| = 4$, \Qbot cannot fully specify attribute values.
    Some example exchanges from the policy learned under this setting are presented in supplement.
}

\noindent
\textbf{Observations.}
\sk{
    Recall the task is an ordered pair of attributes.
    For most tasks, \Qbot learns to \ad{map} them to a pair of tokens in an \emph{order-agnostic fashion}, \ie, both (ordered) tasks for a pair of attributes being represented by the same pair of tokens, while for others it learns compositional encoding.
    For instance, \Qbot groups symmetric tasks (\emph{(color, shape)} and \emph{(shape, color)}), and maps them to an order-agnostic \emph{Y, X}.
    On the other side, tasks \emph{(color, style)} and \emph{(style, color)} \ad{are} encoded as \emph{Z, X} and \emph{X, Z}, respectively.
    At prediction time, \Qbot seems to determine the output order from the task encoding present in its state and simply reorders \Abot's responses as needed.
}

\sk{
    As for the memoryless \Abot, it learns consistent grounding and responds with specific symbols to indicate the inquired attribute, \eg,
    if \Qbot emits $X$ (asks for \emph{color}), \Abot responds with:
    $1 {\rightarrow}$ \emph{blue}, $2 {\rightarrow}$ \emph{purple}, $3 {\rightarrow}$ \emph{green}, $4 {\rightarrow}$ \emph{red}.
    Similar mappings exist for responses to other attributes.
    Essentially, we find the \emph{automatic emergence of grounded language}.
}
\ad{
    Note that this is similar to findings reported in recent works,
    and is most closely related to \cite{visdial_rl}, albeit by taking \Abot's memory away
    rather than \Qbot's state.
}
\FIXME{
-In 4.3, tone down the excitement about emergence of language.
-say that this like recent work, we find language emerges
-this is most similar to the setup of Das et al. ICCV, with the following changes
-we take A`s memory away rather than Q`s state away.}

\sk{
    Notice, however, that a concept can be associated to $a_t = 1$ only if are given the corresponding $q_t$, and $a_t$ cannot be interpreted on its own right.
    For example, $a_t=1$ refers to \emph{blue} when $q_t=X$(\emph{color}), and \emph{triangle} when $q_t=Y$(\emph{shape}).
    Therefore, $a_t=1$ has no absolute grounding \ad{independent of $q_t$}.
    To draw parallels to natural language, although the token `yes' has an affirmative sense,
    complete meaning can be \ad{conveyed} only when we consider the \ad{context -- } preceding question to which `yes' is an answer.
    \eg., `Q: Is it day? A: Yes' and `Q: Is it night? A: Yes' \ad{assigns different meanings to `Yes'} conditioned on question.
    To obtain such absolute token grounding whilst preserving compositionality, one could enforce attribute prediction based only on answers $a_t$ from \Abot, ignoring corresponding questions $q_t$.
    \ad{
        But this is an unintuitive non-human-like setup -- humans use complete QAs to ground concepts.
    }
    % We defer this to future work.
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% experiment did not converge work out of the box
% \subsection{Memoryless \Abot, Memoryless \Qbot}
% \label{sec:toy_alt_task_state}
% \FIXME{Would be nice to get absolute grounding for tokens here. We can talk about it and show this is what obtains grounding. Argue for both sides -- we might not need absolute grounding, give 'Yes' as example and explain. Can push this to supplement in interest of space, experiment still running.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/main/language-chart.tex <==
\vspace{\sectionReduceTop}
\section{Evolution of Language}
\vspace{\sectionReduceBot}

\sk{
    To gain further insights, we visualize partially learned policies at regular intervals during training, via `dialog trees'.
    A dialog tree essentially enumerates all plausible dialogs between the two agents, in the form of a tree.
    At any node, we go deeper by choosing a branch based on the next utterance between these agents ($q_1$ is the root).
    As our \tnt game runs for two rounds, our dialog trees have a depth of $4$ with $|V_A|^2|V_Q|^2$ leaves.
    Notice that an instance could potentially result in different dialogs depending on the task.
    Hence, we consider \emph{(instance, task)} pairs and assign each to a leaf by traversing the tree according to the resulting dialog.
    \reffig{fig:lang_chart} depicts a timeline of concepts learned at various nodes of the trees during training.
    Further details are in the supplement.
}

